Random nilpotent groups, polycyclic presentations, and Diophantine problems

We introduce a model of random f.g., torsion-free, $2$-step nilpotent groups (in short, $\tau_2$-groups). To do so, we show that these are precisely the groups that admit a presentation of the form $ \label{tau2pres_0}\langle A, C \mid [a_i, a_j]= \prod_t {\scriptstyle c_t^{\scriptscriptstyle \lambda_{t,i,j}}} \ (i< j), \ [A,C]=[C,C]=1\rangle,$ where $A=\{a_1, \dots, a_n\}$, and $C=\{c_1, \dots, c_m\}$. Hence, one may select a random $\tau_2$-group $G$ by fixing $A$ and $C$, and then randomly choosing exponents $\lambda_{t,i,j}$ with $|\lambda_{t,i,j}|\leq \ell$, for some $\ell$. We prove that, if $m\geq n-1\geq 1$, then the following holds asymptotically almost surely, as $\ell\to \infty$: The ring of integers $\mathbb{Z}$ is e-definable in $G$, systems of equations over $\mathbb{Z}$ are reducible to systems over $G$ (and hence they are undecidable), the maximal ring of scalars of $G$ is $\mathbb{Z}$, $G$ is indecomposable as a direct product of non-abelian factors, and $Z(G)=\langle C \rangle$. If, additionally, $m \leq n(n-1)/2$, then $G$ is regular (i.e. $Z(G)\leq {\it Is}(G')$). This is not the case if $m > n(n-1)/2$. In the last section of the paper we introduce similar models of random polycyclic groups and random f.g. nilpotent groups of any nilpotency step, possibly with torsion. We quickly see, however, that the latter yields finite groups a.a.s.

==> nonexistence.tex <==

\subsection{Nonexistence of centralizer-small elements}
%
%
\tc{green}{Remove section?}

\tc{teal}{Change introduction. Explain we don't know how is the center when $m\leq (n-1)/2$. Implies we don't know if $G$ has two non-commuting c-small elements. Explain maybe the skew-symmetric thing?} Theorem  \ref{mainthm} relies on the fact that, if $m\geq n-1$, then certain non-commuting c-small elements exist a.a.s. In this section we prove that this is \emph{never} (not only a.a.s.)\ the case  if $m< (n-1)/2$. As explained in the introduction, the intermediate case $(n-1)/2 < m < n-1$ remains open. We also leave open the problem of determining what conclusions from   Theorem \ref{mainthm} still hold when $m<n-1$, a.a.s. 

We start with the following general result, which may be of interest also outside the context of random $\tau_2$-groups. Below, given a subgroup $H$ such that $G'\leq H\leq Z(G)$, we say that an element $g\in G$ is \emph{$H$-c-small} if $C(g)=\{g^tc \mid t\in \mathbb{Z}, \ z\in \C \}.$ %specially when $\C=Z(G)$.
%
\begin{thm}\label{noGP}
%
Let $G$ be a $\tau_2$-group with  Malcev basis $(A;C)$. Suppose that $\rank(G') \leq (\rank(G/\C)-1)/2$. Then $G$ does not have two non-commuting $\C$-c-small elements.  
%
\end{thm}


\begin{proof}
%
Let $n=\rank(G/\C)$ and $m=\rank(G')$. We prove that, under the hypothesis of the lemma, if $a$ and $b$ are two  $\C$-c-small elements of $G$, then $[a,b]=1$.   Let $\phi_a, \phi_b: G/\C \r G'$ be the well-defined homomorphisms $g\C \mapsto [a, g]$ and $g\C \mapsto [b,g]$, respectively, and denote their kernels by  $K_a$ and $K_b$. By hypothesis, $G$ is non-abelian, and thus $G/\C$ and $G'$ are non-trivial. Notice that 
%
\begin{align}\label{Kernels}\left(G/\C\right)/K_a \cong \mbb{Z}^{n}/K_a \cong Im(\phi_a) \leq G' \cong \mbb{Z}^{m}, %\quad \quad \mbb{Z}^{n}/K_b \cong Im(\phi_b) \leq G' \cong \mbb{Z}^{m},
\end{align}
%
and similarly for $\phi_b$ and $K_b$. It follows  that $Im(\phi_a)$ and $Im(\phi_b)$ are free abelian groups, and that $K_b$ and $K_a$ are direct factors of $G/\C \cong \mathbb{Z}^n$. %CCCC\textcolor{gray}{detail?}. Consequently, $G/\C = K_a \times L_a= K_b \times L_b$ for some $L_a$ and $L_b$. 

Next we prove that  $K_a \cap K_b \neq 1.$ First suppose that $\rank(K_a) \leq \rank(L_b).$  By \eqref{Kernels}, $n - \rank(K_a) \leq m$. The same is true for $\rank(K_b)$. Therefore,
%
$$n = \rank(K_b) + \rank(L_b) \geq   \rank(K_b) + \rank(K_a) \geq 2n -2m,$$
%
from where we obtain the  inequality $n/2\leq m$, contradicting the assumption $m\leq (n-1)/2$. 

Now suppose that $\rank(K_a) > \rank(L_b)$, and let  %To tackle this case we will use  Remark \ref{subgroupMatrix} and some well-known properties about Gaussian elimination and subgroups of f.g.\ free abelian groups. Let  
$\mathbf{k}_a, \mathbf{l}_b=\{\ell_i \mid i\},$  $\mathbf{k}_b=\{k_j \mid j\}$ be bases of $K_a, L_b,$ and $K_b,$ respectively. Since $K_a \leq L_b\times K_b$, one may write each $r\in \mathbf{k}_a$ as a linear combination of the elements in $\mathbf{l}_b \cup \mathbf{k}_b$:
%
$$
r=\prod_{i=1}^{|\mathbf{l}_b|} \ell_i^{\alpha_{r,i}} \prod_{j=1}^{|\mathbf{k}_b|} k_j^{\beta_{r,j}}, \quad \alpha_{r,i}, \beta_{r,j}\in \mathbb{Z}.
$$
%
Denote by $M$  the matrix whose set of rows is $$\left\{\left(\alpha_{r,1}, \dots, \alpha_{r,|\mathbf{l}_b|}, \beta_{r,1}, \dots, \beta_{r,|\mathbf{k}_b|}\right) \mid r\in \mathbf{k}_a\right\}$$ (the order of the rows is not important). Notice that if one of these rows starts  with $|\mathbf{l}_b|$ zeros or more, then the corresponding element from $\mathbf{k}_a$ is a linear combination of the basis $\mathbf{k}_b$, and thus $1\neq  K_a \cap K_b$. %\textcolor{gray}{Improve paragraph?}

%As already observed before, 
%$\rank(K_a)=\rank(M)$, and 
As seen in Theorem \ref{regularitythm}, performing row operations on $M$ (interchanging two rows, and adding or subtracting one row to another different row) corresponds to changing the basis $\mathbf{k}_a$ of $K_a$ by means of Nielsen transformations. Therefore, by choosing a new $\mathbf{k}_a$, we may assume that $M$ is in row echelon form, and, in particular, that all entries below the diagonal that starts at the first entry of $M$ are $0$. %Moreover, since $\rank(M)=\rank(K_a)=|\mathbf{k}_a|$ and $M$ has $|\mathbf{k}_a|$ rows, no row of $M$ consists entirely of zeros. 
Under this assumption, the last row  of $M$ starts with $|\mathbf{k}_a|-1 \geq |\mathbf{l}_b|$ zeros. Hence, as noticed above, the last element $r$ of $\mathbf{k}_a$ is equal to a  linear combination of the basis $\mathbf{k}_b$, and thus $1\neq r \in K_a \cap K_b$, as needed.







Take now   a non-trivial element $g\C \in G/\C$ belonging to $K_a \cap K_b$. Then $g$ is a solution to the system $[a, x]=1, \ [b,y]=1$ over $G$. Since $a$ and $b$ are c-small,  $$g=a^{t_a}z_a = b^{t_b}z_b$$ for some  $t_a, t_b\in \mbb{Z}$ and some  $z_a, z_b \in \C$. Plugging this into $1=[a, g] = [g, b]$ we obtain $[a,b]^{t_b} = [a,b]^{t_a}$, and  since $G$ is torsion free, $t_a=t_b=t$. Moreover,  $t\neq 0$ because $g \C$ is non-trivial. But then, using $a^t=b^{t}z_b z_a^{-1}$, $$(ab^{-1})^t = a^t b^{-t} [b^{-1}, a]^{\frac{t(t-1)}{2}} = z_b z_a^{-1} [b^{-1}, a]^{\frac{t(t-1)}{2}} \in \C \leq Z(G).$$  Since $G/Z(G)$ is torsion-free, $ab^{-1} \in Z(G)$, which implies that $[a,b]=1$. This completes the proof of the lemma.
%
\end{proof}




%\begin{remark}
%Following the notation of Theorem \ref{noGP}, we claim that if $g$ is $\C$-c-small and $g\notin Z(G)$, then $\C=Z(G)$. Indeed: suppose there exists $z \in Z(G) \backslash \C$. Then $z\in C(g)$, and hence $z= g^t c$ for some $t\in \mathbb{Z}$ and $c\in \C$. It follows that $g^t\in Z(G)$. Since $G/Z(G)$ is torsion-free, either $t=0$ or $t=1$. But none of these is possible, since $z\notin \C$ and $g\notin Z(G)$, respectively.
%\end{remark}



%Recall that when we introduced the present section \ref{densitySec} we defined $GenP$ (similarly, $Int$) to be the class of $\tau_2$-groups  having two elements in general position (of having two non-commuting c-small elements).
%
%We next apply this result to the setting of random $\tau_2$-groups. 
%
%
%Notice that the following holds \emph{for all} $G$, not only asymptotically almost surely.
%
\begin{cor}\label{noIntegral}
%
Suppose $m\leq (n-1)/2$. Then no group admitting a presentation from $ \mc{P}(n,m)$, as in \eqref{tau2pres2}, has two non-commuting $\C$-c-small elements.
%
\end{cor}
%
\begin{proof}
%
By Corollary \ref{superCor}, $\rank(G')\leq m$, and $(A;C)$ is a  Malcev basis of $G$. Hence, (the projection of) $A$ is a basis of $G/\C$, which implies that $\rank(G/\C)=n$. We obtain  $\rank(G')\leq m\leq (n-1)/2 = (\rank(G/\C) -1 )/2$. The result now follows from Theorem \ref{noGP}.
%
\end{proof}

%



%Following Remark \ref{generalposStrategy}, it might be possible to improve the bound $\mu \geq \s-1$ to $\mu \geq (2\s-1)/3.$ The main obstacle to doing so is the necessity of using normal Malcev bases. First, one needs to prove they always exist, and second,  one may need to slightly modify the current model by requiring that $[a_1, a_2]=c_1.$




%\begin{remark}
%Let $\mbb{Z}$ be the property of having two elements $a,b$ such that $\mc{O}(a,b) =\mbb{Z},$ where $\mc{O}(a,b)$ i as defined in \cite{Part1}. \hlc[lgray]{refer's to Denis' part}. By Propositon \ref{GPimpliesLocalZ} and Theorem \ref{mainThm}, if $\mu \geq \s-1,$ then $$Prob\left(P \in \mc{P}_{\mbb{Z}}(\s, \mu)\right)=1.$$

%\end{remark}
